SAINT: Service-level Integration Test Generation with Program Analysis and LLM-based Agents

Enterprise applications are typically tested at multiple levels, with service-level testing playing an important role in validating application functionality. Existing service-level testing tools, especially for RESTful APIs, often employ fuzzing and/or depend on OpenAPI specifications which are not readily available in real-world enterprise codebases. Moreover, these tools are limited in their ability to generate functional tests that effectively exercise meaningful scenarios. In this work, we present SAINT, a novel white-box testing approach for service-level testing of enterprise Java applications. SAINT combines static analysis, large language models (LLMs), and LLM-based agents to automatically generate endpoint and scenario-based tests. The approach builds two key models: an endpoint model, capturing syntactic and semantic information about service endpoints, and an operation dependency graph, capturing inter-endpoint ordering constraints. SAINT then employs LLM-based agents to generate tests. Endpoint-focused tests aim to maximize code and database interaction coverage. Scenario-based tests are synthesized by extracting application use cases from code and refining them into executable tests via planning, action, and reflection phases of the agentic loop. We evaluated SAINT on eight Java applications, including a proprietary enterprise application. Our results illustrate the effectiveness of SAINT in coverage, fault detection, and scenario generation. Moreover, a developer survey provides strong endorsement of the scenario-based tests generated by SAINT. Overall, our work shows that combining static analysis with agentic LLM workflows enables more effective, functional, and developer-aligned service-level test generation.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\paragraph{Cost of using \tool} One major concern with LLM-based approaches is their operational cost, as excessive token consumption can substantially increase overall expenses and limit practical usage. To evaluate this aspect, we measured the token usage for both endpoint-level and scenario-based test generation, and translated these values into monetary cost using the pricing of different models. Our analysis demonstrates that \tool is significantly cost-efficient, both in terms of total expenditure and the number of LLM invocations. Specifically, with Devstral (via OpenRouter~\cite{openrouter}) the average cost is \$0.24 for endpoint-focused and \$0.22 for scenario-based generation, whereas for o1 (on the OpenAI platform), it is \$6.17 and \$4.42, respectively. The detailed result in present in the supplementary material~\cite{supplementary}. We believe this efficiency primarily because of the integration of static analysis, which enables \tool to perform targeted pre-processing and invoke the LLM only when necessary, rather than feeding the entire application context to an off-the-shelf model.

\vskip -5pt
\paragraph{Benefits and drawbacks of using hybrid approach} Beyond cost, hybrid approaches offer several additional advantages. For example, in terms of HTTP call efficiency, \tool performs significantly fewer requests compared to EvoMaster. On average, \tool issues fewer than 500 HTTP requests per application, whereas EvoMaster generates over 10k+ requests for the same applications, resulting in a more focused and efficient testing process. Another key advantage is scalability—\tool can support major Java versions and frameworks, while conventional tools often struggle to maintain compatibility as the scope expands. Although \tool continues to rely on static analysis, it leverages well-established and actively maintained analysis tools that provide broad language support.

==> model/database.tex <==
\begin{figure}[ht]
\centering

\vspace{0.5em}
% Tuple representation
\[
\mathcal{D} = (F, C, M, L, N, T, O)
\]

\resizebox{\columnwidth}{!}{%
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{>{\bfseries}c @{\hspace{0.8em}} c @{\hspace{0.8em}} p{8cm}}
\toprule
Symbol & Type & Description \\
\midrule
$F$ & $\mathcal{F}$ & Database framework. $\mathcal{F}=\{JDBC, JPA, JTA, ...\}$ \\
$C$ & $\Sigma^*$ & Enclosing class name of the operation \\
$M$ & $\Sigma^*$ & Method signature where the DB access occurs \\
$O$ & $\mathcal{O}$ & CRUD operation type $\mathcal{F}=\{Create, Read, Update, Delete\}$\\
\bottomrule
\end{tabular}
}
\caption{Formal definition of a database access descriptor}
\label{fig:database-tuple}
\end{figure}

==> model/endpoint_parameter.tex <==
\begin{figure}[ht]
\centering

\vspace{0.5em}
% Display the tuple expression
\[
\mathcal{P} = (n, T, K, V, C, M, A)
\]

\resizebox{\columnwidth}{!}{%
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{>{\bfseries}c @{\hspace{0.8em}} c @{\hspace{0.8em}} p{7.5cm}}
\toprule
Symbol & Type & Description \\
\midrule
$n$    & $\Sigma^+$ & Name of the parameter \\
$T$    & $\Sigma^+$ & Datatype (e.g., \texttt{"int"}, \texttt{"str"}) \\
$K$    & $\mathcal{K}$ & Kind of parameter. $\mathcal{K}=\{query, path, body\}$\\
$V$    & $[\Sigma^*]$ & Value constraints (e.g., allowed strings, enum options) \\
$C$    & $\Sigma^*$ & Enclosing class where parameter is defined \\
$M$    & $\Sigma^*$ & Method signature where the parameter is defined \\
$A$    & $[\Sigma^*]$ & List of annotations applied to the parameter \\
\bottomrule
\end{tabular}
}
\caption{Formal definition of an endpoint parameter}
\label{fig:endpoint-parameter}
\end{figure}


==> model/endpoint_path.tex <==
\begin{figure}[ht]
\centering

\vspace{0.5em}
% Tuple expression
\[
\mathbb{P} = (b, p, H)
\]

\resizebox{\columnwidth}{!}{%
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{>{\bfseries}c @{\hspace{0.8em}} c @{\hspace{0.8em}} p{8cm}}
\toprule
Symbol & Type & Description \\
\midrule
$b$ & $\Sigma^*$ & Base path prefix shared across endpoints in the class \\
$p$ & $\Sigma^*$ & Path specific to the endpoint method \\
$H$ & $\mathbb{H}$ & HTTP method. $\mathbb{H}=\{GET, POST, PUT, DELETE, PATCH\}$\\
\bottomrule
\end{tabular}
}
\caption{Formal definition of an endpoint path}
\label{fig:method-endpoint-path}
\end{figure}

==> model/ipd.tex <==
\begin{figure}[ht]
\centering

\vspace{0.5em}
% Display the tuple representation
\[
\mathcal{I} = (R, \Pi, \Gamma)
\]

\resizebox{\columnwidth}{!}{%
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{>{\bfseries}c @{\hspace{0.8em}} c @{\hspace{0.8em}} p{8cm}}
\toprule
Symbol & Type & Description \\
\midrule
$R$       & $\Sigma^*$ & Relation type (e.g., \texttt{"AllOrNone"}, \texttt{"Requires"}, \texttt{"OnlyOne"}, etc.) \\
$\Pi$     & $[\mathcal{P}]$ & List of involved parameters\\
$\Gamma$  & $\Sigma^*$ & Constraint logic associated with the relation (e.g., string expression or rule description) \\
\bottomrule
\end{tabular}
}
\caption{Formal definition of an inter-parameter dependency}
\label{fig:abstract-ipd}
\end{figure}

==> tables/model.tex <==
% \begin{table}[h!]
% \centering
% \renewcommand{\arraystretch}{1.0}
% \resizebox{0.8\linewidth}{!}{
% \begin{tabular}{c|c|c|c|c}
% \shortstack{\textbf{Model}} & 
% \shortstack{\textbf{Organization}} & 
% \shortstack{\textbf{Family}} & 
% \shortstack{\textbf{Size} } & 
% \shortstack{\textbf{Open} \\ \textbf{Source?}} \\
% \hline
% \hline
% Granite-3.1-8b & IBM & Granite & 8B & \textcolor{teal}{\textbf{\checkmark}} \\
% \hline
% Llama-3.1-8b & Meta & Llama & 8B & \textcolor{teal}{\textbf{\checkmark}} \\
% \hline
% DeepSeek-R1-Distill-Qwen-32B & DeepSeek & DeepSeek & 32B & \textcolor{teal}{\textbf{\checkmark}} \\
% \hline
% Devstral-small & Mistral & Devstral & 25B & \textcolor{teal}{\textbf{\checkmark}} \\
% \hline
% o1 & OpenAI &GPT & 1T & \textcolor{red}{\textbf{X}} \\
% \hline
% % Claude 3.7 Sonnet & Anthropic & Claude & 1T & \textcolor{red}{\textbf{X}} \\
% % \hline

% \end{tabular}}
% \vspace{1em}
% \caption{Model characteristics}
% \label{tb:model}
% \end{table}


==> tb-prompt.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
% Table generated by Excel2LaTeX from sheet 'Sheet6'
\begin{table*}[htbp]
  \centering
  \caption{Prompt description}
  \begin{minipage}{\linewidth}
  \small
    \begin{tabular}{p{3.1cm}|l|l|p{4.4cm}|p{2cm}|p{2cm}|}
    % \line
    Prompt Name & \multicolumn{1}{l|}{Usage Stage} & \multicolumn{1}{l|}{Description} & Required Parameters & Optional Parameters & Output format \\
    \hline
    Parameter type extraction &       &       & 1. Parameter names\newline{}2. Relevant method bodies & \multicolumn{1}{l|}{} & {<parameter\_name>:<type>} \\
    \hline
    IPD Extraction &       &       & 1. IPD definition\newline{}2. IPD examples\newline{}3. Parameter names\newline{}4. Relevant method bodies & \multicolumn{1}{l|}{} & [{"relation\_type":<>, "parameters": [<list of parameters>]},] \\
    \hline
    Value constraint extraction &       &       & 1. Parameter name and types\newline{}2. Relevant method bodies & 1. ORM fields including types & {<parameter\_name>:[<constraints>,]} \\
    \hline
    Parameter value generation &       &       & 1. Parameter name\newline{}2. Parameter type\newline{}3. IPD\newline{}4. IPD definition\newline{}5. Value constraint & 1. ORM code and field details\newline{}2. Login pattern\newline{} & [ {<parameter>: <value>,...},] \\
    \hline
    Agent planning &       &       & 1. parameter name, type, IPD, constraints\newline{}2. tool choice definition\newline{} & 1. Previous successful requests associated with the endpoint\newline{}2. Erroneous requests\newline{}3. Uncovered code & [{"choice": <tool\_choice>, "explanation": "..."}, ] \\
    \hline
    Agent reflection &       &       & 1. Solution progress report & 1. Uncovered code before actions\newline{}2. Original erroneous HTTP request summary & [{"score": <score action> , "reflection": <reflection summary> }, ] \\
    \hline
    Agent progress summary &       &       & \multicolumn{1}{l|}{} & 1. Uncovered code before and after actions\newline{}2. HTTP response summaries before and after actions & <Summary> \\
    \hline
    TU: Parameter type modification &       &       & \multirow{5}[10]{*}{1. Parameter names\newline{}2. Relevant method bodies} & \multirow{5}[10]{*}{1. ORM code and field details\newline{}2. Uncovered code\newline{}3. Erroneous request\newline{}4. Additional code context from code context action\newline{}5. Choice explanation} & {<parameter\_name>:<type>} \\
\cline{1-3}\cline{6-6}    TU: Parameter value modification &       &       & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & [ {<parameter>: <value>,...},] \\
\cline{1-3}\cline{6-6}    TU: IPD modification &       &       & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & [{"relation\_type":<>, "parameters": [<list of parameters>]},] \\
\cline{1-3}\cline{6-6}    TU: Generate more requests &       &       & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & [ "endpoint\_name": [{<parameter>: <value>,...},]] \\
\cline{1-3}\cline{6-6}    TU: Update value constraints &       &       & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & {<parameter\_name>:[<constraints>,]} \\
    \hline
    TU: Code context extraction &       &       & 1. CLDK API details\newline{}2. Relevant code & \multicolumn{1}{l|}{} & CLDK API \\
    \hline
    HTTP response summarization &       &       & 1.HTTP Response & \multicolumn{1}{l|}{} & <Summary> \\
    \hline
    Endpoint operation summarization &       &       & 1. Endpoint class name\newline{}2. Endpoint method name\newline{}3. Relevant code for each endpoint & \multicolumn{1}{l|}{} & [<endpoint\_details>:<operation\_summary>] \\
    \hline
    Scenario generation &       &       & 1. Endpoint class name\newline{}2. Endpoint method name\newline{}3. Operation summary & \multicolumn{1}{l|}{} & [{"scenario\_name":<name>,  "given\_description": <description>, "when\_description":<description>, "then\_description":<description>},…] \\
    \hline
    Endpoint sequence generation &       &       & 1. Endpoint class names\newline{}2. Endpoint method names\newline{}3. Scenario details & \multicolumn{1}{l|}{} & {"given\_endpoints":[<endpoint\_details>], "when\_endpoints":[<endpoint\_details>], "then\_endpoints":[<endpoint\_details>]} \\
    \hline
    Endpoint sequence parameter value generation &       &       & 1. Parameter name\newline{}2. Parameter type\newline{}3. IPD\newline{}4. IPD definition\newline{}5. Value constraint\newline{}6. Scenario details & 1. ORM code and field details\newline{}2. Login pattern\newline{} & [ "endpoint\_name": [{<parameter>: <value>,...},]] \\
    \bottomrule
    \end{tabular}%
    \end{minipage}
  \label{tab:addlabel}%
\end{table*}%


% \begin{table*}[htbp]
%   \centering
%   \caption{Prompt description}
%   \begin{minipage}{\linewidth}
%   \small
%     \begin{tabular}{|r|l|c|r|r|r|r|}
%     \hline
%     \multicolumn{1}{|c|}{Sl No} & \multicolumn{1}{c|}{Name} & \multicolumn{1}{c|}{Stage} & \multicolumn{1}{c|}{Required parameters} & \multicolumn{1}{c|}{Optional parameters} & \multicolumn{1}{c|}{Output format} & \multicolumn{1}{c|}{Description} \\
%     \hline
%     \hline
%     1     & Extract parameter type  &   \circled{4}    &       &       &  \\
%     \hline
%     2     & Extract inter-parameter dependencies &    \circled{5}    &       &       &       &  \\
%     \hline
%     3     & Extract value constraints &   \circled{6}     &       &       &       &  \\
%     \hline
%     4     & Login pattern &  \circled{8}      &       &       &       &  \\
%     \hline
%     5     & Parameter value generation &   \circled{8}    &       &       &       &  \\
%     \hline
%     6     & HTTP request fixing agent planning phase &    \circled{10}    &       &       &       &  \\
%     \hline
%     7     & HTTP response summarization &    \circled{10}    &       &       &       &  \\
%     \hline
%     8     & HTTP request fixing agent progress summary &  \circled{10}      &       &       &       &  \\
%     \hline
%     9     & HTTP request fixing agent reflection phase &    \circled{10}    &       &       &       &  \\
%     \hline
%     10    & Coverage augmentation agent planning phase &   \circled{11}     &       &       &       &  \\
%     \hline
%     11    & Coverage augmentation agent progress summary &   \circled{11}     &       &       &       &  \\
%     \hline
%     12    & Coverage augmentation agent reflection phase &   \circled{11}     &       &       &       &  \\
%     \hline
%     13    & Tool usage: parameter type modification &  \circled{10} \& \circled{11}       &       &       &       &  \\
%     \hline
%     14    & Tool usage: parameter path modification &   \circled{10} \& \circled{11}    &       &       &       &  \\
%     \hline
%     15    & Tool usage: parameter value modification &   \circled{10} \& \circled{11}    &       &       &       &  \\
%     \hline
%     16    & Tool usage: exercise other endpoint as priori &    \circled{10} \& \circled{11}   &       &       &       &  \\
%     \hline
%     17    & Tool usage: get additional code context &   \circled{10} \& \circled{11}    &       &       &       &  \\
%     \hline
%     18    & Endpoint process sequence generation &   \circled{1}   &       &       &       &  \\
%     \hline
%     19    & Scenario generation &   \circled{13}    &       &       &       &  \\
%     \hline
%     20    & Endpoint operation summary generation &    \circled{14}    &       &       &       &  \\
%     \hline
%     \end{tabular}%
%     \end{minipage}
%   \label{tb:prompts}%
% \end{table*}%

